From Classification to Generation: Insights into Crosslingual Retrieval Augmented ICL

The remarkable ability of Large Language Models (LLMs) to understand and follow instructions has sometimes been limited by their in-context learning (ICL) performance in low-resource languages. To address this, we introduce a novel approach that leverages cross-lingual retrieval-augmented in-context learning (CREA-ICL). By extracting semantically similar prompts from high-resource languages, we aim to improve the zero-shot performance of multilingual pre-trained language models (MPLMs) across diverse tasks. Though our approach yields steady improvements in classification tasks, it faces challenges in generation tasks. Our evaluation offers insights into the performance dynamics of retrieval-augmented in-context learning across both classification and generation domains.

==> Limitation.tex <==
While our study has yielded promising results, it is not without limitations. The effectiveness of retrieval augmentation is also tied to the model architecture, and its impact on different models remains largely unexplored. In addition, the availability of specific language datasets for sentence retrieval and resource constraints remain practical challenges. Further exploration of prompt design and consideration of external factors could improve our methodology. Acknowledging these limitations is essential for a full interpretation of our results and the direction of future research.

==> validation.tex <==
% don't forget that when the prediction doesn't belong to labels, it will be taken as one of the labels: task1-0, task2-negative

\begin{table}[]
\begin{tabular}{|lrrrrrrrr|}
\hline
\multicolumn{1}{|l|}{}                          & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1}    & \multicolumn{1}{c|}{Accuracy}       & \multicolumn{1}{c|}{Precision}       & \multicolumn{1}{c|}{Recall}      & \multicolumn{1}{c|}{F1}      \\ \hline
\multicolumn{9}{|l|}{bloomz-3b}                                                                                                                                                                                                                                                                                            \\ \hline
\multicolumn{1}{|l|}{}                          & \multicolumn{4}{c|}{"Does the following sentence represent Direct Violence, Passive Violence, or Non-Violence? \{text\}"} & \multicolumn{4}{c|}{'The nature of the text "\{text\}" is most likely: (Direct Violence, Passive Violence, Non-Violence). Please identify.'} \\ \hline
\multicolumn{1}{|l|}{zero shot}                 & \multicolumn{1}{r|}{48.05}    & \multicolumn{1}{r|}{31.67}     & \multicolumn{1}{r|}{48.05}  & \multicolumn{1}{r|}{28.11} & \multicolumn{1}{r|}{53.76}          & \multicolumn{1}{r|}{47.69}           & \multicolumn{1}{r|}{53.76}       & 30.27                        \\ \hline
\multicolumn{1}{|l|}{bangla-template zero shot} & \multicolumn{1}{r|}{53.91}    & \multicolumn{1}{r|}{29.06}     & \multicolumn{1}{r|}{53.91}  & \multicolumn{1}{r|}{23.35} & \multicolumn{1}{r|}{53.91}          & \multicolumn{1}{r|}{29.06}           & \multicolumn{1}{r|}{53.91}       & 23.35                        \\ \hline
\multicolumn{1}{|l|}{main-1}                    & \multicolumn{1}{r|}{53.23}    & \multicolumn{1}{r|}{32.79}     & \multicolumn{1}{r|}{53.23}  & \multicolumn{1}{r|}{26.01} & \multicolumn{1}{r|}{53.91}          & \multicolumn{1}{r|}{29.06}           & \multicolumn{1}{r|}{53.91}       & 23.35                        \\ \hline
\multicolumn{1}{|l|}{main-3}                    & \multicolumn{1}{r|}{53.38}    & \multicolumn{1}{r|}{32.02}     & \multicolumn{1}{r|}{53.38}  & \multicolumn{1}{r|}{24.47} & \multicolumn{1}{r|}{53.83}          & \multicolumn{1}{r|}{29.07}           & \multicolumn{1}{r|}{53.83}       & 23.34                        \\ \hline
\multicolumn{9}{|l|}{mbert}                                                                                                                                                                                                                                                                                                \\ \hline
\multicolumn{1}{|l|}{}                          & \multicolumn{4}{l|}{{[}MASK{]} violence: \{text\}}                                                                        & \multicolumn{4}{l|}{\{text\} this text is {[}MASK{]} violence.}                                                                              \\ \hline
\multicolumn{1}{|l|}{zero shot}                 & \multicolumn{1}{r|}{36.61}    & \multicolumn{1}{r|}{37.16}     & \multicolumn{1}{r|}{36.61}  & \multicolumn{1}{r|}{30.78} & \multicolumn{1}{r|}{16.54}          & \multicolumn{1}{r|}{86.17}           & \multicolumn{1}{r|}{16.54}       & 11.72                        \\ \hline
\multicolumn{1}{|l|}{main-1}                    & \multicolumn{1}{r|}{40.30}    & \multicolumn{1}{r|}{55.37}     & \multicolumn{1}{r|}{40.30}  & \multicolumn{1}{r|}{25.62} & \multicolumn{1}{r|}{15.78}          & \multicolumn{1}{r|}{93.54}           & \multicolumn{1}{r|}{15.78}       & 10.31                        \\ \hline
\multicolumn{1}{|l|}{main-3}                    & \multicolumn{1}{r|}{40.82}    & \multicolumn{1}{r|}{57.11}     & \multicolumn{1}{r|}{40.82}  & \multicolumn{1}{r|}{25.31} & \multicolumn{1}{r|}{14.81}          & \multicolumn{1}{r|}{98.89}           & \multicolumn{1}{r|}{14.81}       & 8.74                         \\ \hline
\end{tabular}
\caption{results (F1 is macro F1 score) of task1 valid with bloomz-3b and mbert}
\label{tab:results F1 is macro F1 score of task1 valid with bloomz-3b and mbert}
\end{table}


\begin{table}[]
\begin{tabular}{lrrrrrrrrrrrr}
        & \multicolumn{4}{l}{with 1 sample}                                                                                  & \multicolumn{4}{l}{with 3 sample}                                                                                  & \multicolumn{4}{l}{with 5 sample}                                                                                  \\
        & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} \\
\multicolumn{13}{l}{retrieval similar sample}                                                                                                                                                                                                                                                                                                                          \\
english & 58.13                        & 49.57                         & 58.13                      & 58.13                  & 58.41                        & 49.34                         & 58.41                      & 58.41                  & 57.83                        & 48.71                         & 57.83                      & 57.83                  \\
self    & 58.87                        & 49.94                         & 58.87                      & 58.87                  & 58.52                        & 50.00                         & 58.52                      & 58.52                  & 57.30                        & 49.48                         & 57.30                      & 57.30                  \\
\multicolumn{13}{l}{random sample}                                                                                                                                                                                                                                                                                                                                     \\
english & 56.94                        & 50.00                         & 56.94                      & 56.94                  & 56.66                        & 49.18                         & 56.66                      & 56.66                  & 56.33                        & 48.79                         & 56.33                      & 56.33                  \\
self    & 53.46                        & 49.77                         & 53.46                      & 53.46                  & 53.00                        & 50.41                         & 53.00                      & 53.00                  & 50.03                        & 49.06                         & 50.03                      & 50.03                  \\
\multicolumn{13}{l}{samples per label-retrieval similar sample}                                                                                                                                                                                                                                                                                                        \\
english & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}   & 57.02                        & 49.35                         & 57.02                      & 57.02                  & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}   \\
\multicolumn{13}{l}{samples per label-random sample}                                                                                                                                                                                                                                                                                                                   \\
english & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}   & 55.19                        & 51.07                         & 55.19                      & 55.19                  & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}  
\end{tabular}
\caption{results (F1 is micro F1 score) of task2 valid with bloomz-3b model using english and bangla(self, :10000 of train) retrieval dataset, prompt template:"Classify the text as one of the following sentiments:Positive, Negative, or Neutral\textbackslash{}n\textbackslash{}nText:\{text\}\textbackslash{}nSentiment:"}
\label{tab:results F1 is micro F1 score of task2 valid with bloomz-3b model using english and banglaself :10000 of train retrieval dataset}
\end{table}



\begin{table}[]
\begin{tabular}{lrrrrrrrrrrrr}
                                                                                                      & \multicolumn{4}{l}{zero shot}                                                                                      & \multicolumn{4}{l}{with 1 sample}                                                                                  & \multicolumn{4}{l}{with 3 sample}                                                                                  \\
                                                                                                      & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} \\
pattern 0: \{text\} {[}MASK{]}                                                                        & 23.38                        & 69.49                         & 23.38                      & 23.38                  & 32.02                        & 42.81                         & 32.02                      & 32.02                  & 32.35                        & 42.71                         & 32.35                      & 32.35                  \\
pattern 1: {[}MASK{]}: \{text\}                                                                       & 32.23                        & 48.06                         & 32.23                      & 32.23                  & 36.50                        & 40.22                         & 36.50                      & 36.50                  & 40.08                        & 44.13                         & 40.08                      & 40.08                  \\
pattern 2: {[}MASK{]} text: \{text\}                                                                  & 29.20                        & 51.96                         & 29.20                      & 29.20                  & 37.41                        & 41.00                         & 37.41                      & 37.41                  & 40.82                        & 45.07                         & 40.82                      & 40.82                  \\
pattern 3: \{text\} Sentiment: {[}MASK{]}                                                             & 33.68                        & 44.64                         & 33.68                      & 33.68                  & 38.38                        & 41.48                         & 38.38                      & 38.38                  & 40.87                        & 43.57                         & 40.87                      & 40.87                  \\
pattern 4: \{text\} What is a possible sentiment for the text given the following options: {[}MASK{]} & 38.10                        & 63.58                         & 38.10                      & 38.10                  & 35.23                        & 42.13                         & 35.23                      & 35.23                  & 37.31                        & 40.64                         & 37.31                      & 37.31                  \\
pattern 5: \{text\} Classify the sentiment of this text as Positive, Negative, or Neutral: {[}MASK{]} & 43.69                        & 92.41                         & 43.69                      & 43.69                  & 34.57                        & 40.67                         & 34.57                      & 34.57                  & 37.51                        & 40.07                         & 37.51                      & 37.51                  \\
pattern 6: \{text\} In summary, the sentiment is {[}MASK{]}                                           & 44.38                        & 58.36                         & 44.38                      & 44.38                  & 35.94                        & 42.11                         & 35.94                      & 35.94                  & 38.76                        & 41.21                         & 38.76                      & 38.76                  \\
pattern 7: \{text\} the possible sentiment for the text given the following options is {[}MASK{]}     & 35.46                        & 98.47                         & 35.46                      & 35.46                  & 37.77                        & 42.15                         & 37.77                      & 37.77                  & 40.59                        & 42.06                         & 40.59                      & 40.59                  \\
pattern 8: \{text\} the sentiment of this text as Positive, Negative, or Neutral is {[}MASK{]}        & 43.44                        & 74.14                         & 43.44                      & 43.44                  & 34.79                        & 43.15                         & 34.79                      & 34.79                  & 36.57                        & 41.36                         & 36.57                      & 36.57                  \\
                                                                                                      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}   & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}   & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}  
\end{tabular}
\caption{results of mbert in task2 valid with different templates}
\label{tab:results of mbert in task2 valid with different templates}
\end{table}


\begin{table}[]
\begin{tabular}{|lrrrrrrrrrrrr|}
\hline
\multicolumn{1}{|l|}{}          & \multicolumn{4}{l|}{zero shot}                                                                                            & \multicolumn{4}{l|}{with 1 sample}                                                                                        & \multicolumn{4}{l|}{with 3 sample}                                                                                     \\ \hline
\multicolumn{1}{|l|}{}          & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1}    & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1}    & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1} \\ \hline
\multicolumn{13}{|l|}{bloom-3b, "Text:\{text\} What is a possible sentiment for the text given the following options?"}                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{1}{|l|}{}          & \multicolumn{1}{r|}{44.56}    & \multicolumn{1}{r|}{19.86}     & \multicolumn{1}{r|}{44.56}  & \multicolumn{1}{r|}{44.56} & \multicolumn{1}{r|}{44.56}    & \multicolumn{1}{r|}{19.86}     & \multicolumn{1}{r|}{44.56}  & \multicolumn{1}{r|}{44.56} & \multicolumn{1}{r|}{44.56}    & \multicolumn{1}{r|}{19.86}     & \multicolumn{1}{r|}{44.56}  & 44.56                   \\ \hline
\multicolumn{13}{|l|}{bloomz-3b, main method}                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|l|}{template0} & \multicolumn{1}{r|}{61.54}    & \multicolumn{1}{r|}{50.83}     & \multicolumn{1}{r|}{61.54}  & \multicolumn{1}{r|}{61.54} & \multicolumn{1}{r|}{58.41}    & \multicolumn{1}{r|}{49.34}     & \multicolumn{1}{r|}{58.41}  & \multicolumn{1}{r|}{58.41} & \multicolumn{1}{r|}{57.83}    & \multicolumn{1}{r|}{48.71}     & \multicolumn{1}{r|}{57.83}  & 57.83                   \\ \hline
\multicolumn{1}{|l|}{template5} & \multicolumn{1}{r|}{61.06}    & \multicolumn{1}{r|}{48.80}     & \multicolumn{1}{r|}{61.06}  & \multicolumn{1}{r|}{61.06} & \multicolumn{1}{r|}{57.80}    & \multicolumn{1}{r|}{50.50}     & \multicolumn{1}{r|}{57.80}  & \multicolumn{1}{r|}{57.80} & \multicolumn{1}{r|}{58.64}    & \multicolumn{1}{r|}{54.89}     & \multicolumn{1}{r|}{58.64}  & 58.64                   \\ \hline
\multicolumn{13}{|l|}{bangla template}                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
\multicolumn{1}{|l|}{template0} & \multicolumn{1}{r|}{58.67}    & \multicolumn{1}{r|}{49.33}     & \multicolumn{1}{r|}{58.67}  & \multicolumn{1}{r|}{58.67} & \multicolumn{1}{r|}{}         & \multicolumn{1}{r|}{}          & \multicolumn{1}{r|}{}       & \multicolumn{1}{r|}{}      & \multicolumn{1}{r|}{}         & \multicolumn{1}{r|}{}          & \multicolumn{1}{r|}{}       &                         \\ \hline
\multicolumn{1}{|l|}{template5} & \multicolumn{1}{r|}{44.94}    & \multicolumn{1}{r|}{55.21}     & \multicolumn{1}{r|}{44.94}  & \multicolumn{1}{r|}{44.94} & \multicolumn{1}{r|}{}         & \multicolumn{1}{r|}{}          & \multicolumn{1}{r|}{}       & \multicolumn{1}{r|}{}      & \multicolumn{1}{r|}{}         & \multicolumn{1}{r|}{}          & \multicolumn{1}{r|}{}       &                         \\ \hline
\multicolumn{13}{|l|}{hindi retrieval dataset}                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|l|}{template0} & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}      & \multicolumn{1}{r|}{53.33}    & \multicolumn{1}{r|}{50.65}     & \multicolumn{1}{r|}{53.33}  & \multicolumn{1}{r|}{53.33} & \multicolumn{1}{r|}{54.30}    & \multicolumn{1}{r|}{50.41}     & \multicolumn{1}{r|}{54.30}  & 54.30                   \\ \hline
\multicolumn{1}{|l|}{template5} & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}      & \multicolumn{1}{r|}{55.47}    & \multicolumn{1}{r|}{46.51}     & \multicolumn{1}{r|}{55.47}  & \multicolumn{1}{r|}{55.47} & \multicolumn{1}{r|}{56.46}    & \multicolumn{1}{r|}{46.88}     & \multicolumn{1}{r|}{56.46}  & 56.46                   \\ \hline
\end{tabular}
\caption{results of two templates in task2 valid of different lines, one bloom-3b, others are bloomz-3b. We use template 0 for "Classify the sentiment of this text as Positive, Negative, or Neutral? \textbackslash{}nText:\{text\}\textbackslash{}nSentiment:", which is used before with english and bengla retrieval dataset. And template 5 for "Text:\{text\} What is a possible sentiment for the text given the following options?", which is used at the end of test.}
\label{tab:results of two templates in task2 valid}
\end{table}



